Stein Variational Gradient Descent With Matrix-Valued Kernels

Stein variational gradient descent (SVGD) is a particle-based inference algorithm that leverages gradient information for efficient approximate inference. In this work, we enhance SVGD by leveraging preconditioning matrices, such as the Hessian and Fisher information matrix, to incorporate geometric information into SVGD updates. We achieve this by presenting a generalization of SVGD that replaces the scalar-valued kernels in vanilla SVGD with more general matrix-valued kernels. This yields a significant extension of SVGD, and more importantly, allows us to flexibly incorporate various preconditioning matrices to accelerate the exploration in the probability landscape. Empirical results show that our method outperforms vanilla SVGD and a variety of baseline approaches over a range of real-world Bayesian inference tasks.

==> tex/matrix_svgd.tex <==
\section{Matrix-valued Kernels}
\paragraph{RKHS}
Given a positive definite kernel $k(x, x^\prime): \X \times \X \rightarrow \R, \X\in \R^d$, 
it uniquely defines a reproducing kernel Hilbert space (RKHS) $\H$, 
which is the 
%For $d=1$, $\H^1$ is a real-valued RKHS formed by the 
closure of functions of form $f(x)=\sum_{\ell} a_{\ell} k(x, x^\ell)$ where $a_\ell \in \R$, %$m \in \mathbb{N}$, 
equipped with an inner product 
$\langle f, g\rangle_{\H^d} = \sum_{\ell,\ell^\prime} a_\ell k(x^\ell, x^{\ell^\prime})b_{\ell^\prime}$ for $g(x)=\sum_{\ell^\prime} b_{\ell^\prime} k(x, x^{\ell^\prime})$. 
%Consider $d>1$, $\H^d$ is now a product of real-valued RKHS 
Given a set of positive definite kernels $k_i(x,x')$ and their RKHS $\H_i$, 
consider the product space $\H = \H_1 \times \H_2 \cdots \times \H_d$ 
consisting of 
% vector-valued 
functions of form ${f}=[f_1,\cdots, f_d]^\top$ with $f_i\in \H_i$.
For any function ${f}$ and ${g}$ in $\H$, their inner product and the corresponding norm are defined by
$$
\langle {f},{g} \rangle_{\H} = \sum_{i=1}^d \langle f_i, g_i \rangle_{\H_i},  ~~~
||{f}||_{\H} = \sqrt{\sum_{i=1}^d ||f_i||_{\H_i}^2}.
$$

\paragraph{Matrix-valued Kernel}
$\kk$ is a matrix-valued function, the value of $\kk(x, x')$ is a $d-\mathrm{by}-d$ matrix.

$\H_{\kk}$ is a vector-valued RKHS generated by the kernel function $\kk$.
The kernel function is positive in the sense that xxxx.

\section{Matrix SVGD}
Let $k$ be a scalar kernel funciton and $L$ be an $d\times d$ positive semi-definite matrix.
Then the function $\kk(x,x') =k(x,x')L$ is  positive and hence defined a matrix-valued kernel.


\section{SVGD with Separable Matrix-valued Kernels}


There are many different matrix-valued kernel in literature,
We first consider the most simple separable kernels:
\begin{pro}
When matrix kernel is a separable kernel where $K(x,x') = k(x,x')B$, with scalar kernel $k(x,x')$ and 
B is a positive semi-definite matrix,
we will have our SVGD direction:
\begin{align*}
    % & \E_{x'\sim q}[B k(x,x')\nabla \log p(x') + \sum_{i=1}^D \frac{\partial k(x,x')B e_i}{\partial x'_i}]] \\
    \phi_K^*(\cdot) =& B \E_{x\sim q}[k(x,\cdot)\nabla \log p(x) + \nabla_{x} k(x,\cdot)] \\
    =& B \phi_k^*(\cdot).
\end{align*}
where $\phi_k^*(\cdot)$ is the vanilla SVGD direction when we apply on RKHS with each dimension with the same scalar kernel $k$.
\label{pro:sep_svgd}
\end{pro}






==> tex/method.tex <==
\section{SVGD with matrix-valued kernel}
In this section, we present our result for matrix-valued SVGD.

KSD, xxx

We first start with our main result on SVGD direction on a general matrix-valued kernel $\kk$:
\begin{thm}
For a general matrix kernel $\kk(x,x')$, the SVGD direction is:
\begin{equation}
    \ff_{\kk}^*(\cdot) = \E_{x\sim q}[\kk(x,\cdot)\nabla_{x} \log p(x) + \sum_{i=1}^d \frac{\partial \kk(x,\cdot)e_i}{\partial x_i}],
\label{equ:matrix_svgd}
\end{equation}
where $e_i$ is a unit vector with coefficient $1$ at the $i^{\text{th}}$ coordinate and $x_i$ is the coefficient at the $i^{\text{th}}$ coordinate of $x$. 
\label{pro:matrix_svgd}
\end{thm}
There are mainly two parts of the matrix SVGD direction, similar to original SVGD.
One part is a weighted average for gradient over $\log p(x)$, with a matrix value kernel $\kk(x,\cdot)$ on the left side.
The other part is an gradient operator over the matrix kernel $\kk$. We can see inside the summation, $\kk(x,\cdot)e_i$ is a vector and $x_i$ is a scalar, so the partial derivative can be seen as a vector.

\paragraph{Compared with vanilla SVGD}
If we let $\kk(x,y) = k(x,y)\textbf{I}_D$, with $\textbf{I}_D$ as a $D\times D$ identity matrix, we can see that with this special matrix kernel we can reduce the direction back to the original SVGD direction. 
Now we need to design our matrix kernel to see if we can outperform the original SVGD after a carefully design of a matrix kernel.

\subsection{Separable Matrix-valued Kernels}
The most simple matrix kernel we first come up with is separable kernel, where we can view it as a scalar kernel $k$ times a PSD matrix $B$.
The SVGD direction for this kernel can be calculated using the following proposition.
\begin{pro}
When matrix kernel is a separable kernel where $\kk(x,x') = k(x,x')B$, with scalar kernel $k(x,x')$ and 
a positive semi-definite matrix B,
we will have SVGD direction:
\begin{align}
    % & \E_{x'\sim q}[B k(x,x')\nabla \log p(x') + \sum_{i=1}^D \frac{\partial k(x,x')B e_i}{\partial x'_i}]] \\
    \ff_\kk^*(\cdot) =& B \E_{x\sim q}[k(x,\cdot)\nabla \log p(x) + \nabla_{x} k(x,\cdot)] \nonumber \\
    =& B \phi_k^*(\cdot).
\label{equ:seq_svgd}
\end{align}
where $\ff_k^*(\cdot)$ is the original SVGD direction with the same scalar kernel $k$ in each dimension.
\label{pro:sep_svgd}
\end{pro}
We can see that with a separable kernel, our SVGD direction is just the original direction left times a PSD matrix $B$.
\paragraph{Connection with Stein Newton's method}
In unconstrained optimization, there is a basic method called line search.
There are usually two ways to compute the descent direction: one is first order based method, like gradient descent; the other is second order based method, like Newton's method and Quasi Newton's.
If we think vanilla SVGD is a gradient based method, by left times a PSD matrix including second order information, we can view SVGD with separable matrix kernel as a (Quasi) Newton's method.

An interesting PSD matrix we can apply here is to follow \cite{detommaso2018stein}.
The matrix is actually an inverse from sum of two matrices. 
One is the Hessian of logarithmic of our target density function, $\nabla^2 \log p(x)$. 
The other one is from the Hessian of the kernel, $\nabla^2 k(x,\cdot)$.
As we can see, if we take the average Hessian kernel, both matrices is approximately proportional to:
$$M_p = \E[\nabla^2 \log p(x)].$$
To design a separable matrix kernel, we could let $B = M_p^{-1}$ to take the advantage of Newton's acceleration.

\paragraph{Linear transformation of random variables}
Another point of view for understanding the above matrix kernel with separable matrix $B = M_p^{-1}$ is by linear transformation of random variables.

To simplify the problem and get intuition, let say our goal distribution $p$ is a Gaussian with covariance matrix $\Sigma$.
We know that an standard Normal distribution can be learned by vanilla SVGD using RBF kernel, where
$$k_{\text{RBF}}(x,x') = \exp\bigg\{-\|x-x'\|^2/2h\bigg\},$$
and its corresponding matrix kernel can be written as:
$$\kk = k_{\text{RBF}}\textbf{I}_D.$$

Suppose $\{x^{(i)}\}_{i=1}^n$ is the set of particles we evolve using vanilla SVGD.
Now considering particles $y = Ax + b$. 
If the original particles can approximate standard normal distribution, then $y$ can approximate $\N(b, \Sigma)$ with $\Sigma = AA^T$.

The SVGD direction for x based on matrix kernel $\kk_x$ would be 
$$\phi_{\kk_x}^*(\cdot) \propto \hat{\E}_{x}[\stein_{p_x}\kk_x(x,\cdot)],$$
and if we update $y$ based on the update for $x$ we have
$$y^{new} = Ax^{new} + b = A(x+\epsilon \phi_{\kk_x}^*(x)) + b = y + \epsilon A\phi_{\kk_x}^*(x).$$

% We only need to see how to update $x$, and the relation if we change of variable to y.

Since 
$$\stein_{p_X}\kk(x,\cdot) = \kk(x,\cdot)\nabla_x \log p_X(x) + \sum_{i=1}^d \frac{\partial \kk(x,\cdot)e_i}{\partial x_i},$$
consider $\nabla_x \log p_X(x).$
If $y = Ax + b$, $y\sim p_Y$ satisfies $p_Y(y) = |det(\frac{dx}{dy})|p_X(x) = |det(A^{-1}|p_X(x)$. Thus,
\begin{align*}
    \nabla_x \log p_X(x) =& (\frac{\partial \log p_X(x)}{\partial x_i})_{i=1}^d\\
    =& (\sum_{j=1}^d \frac{\partial \log p_X(x)}{\partial y_j}\frac{\partial y_j}{\partial x_i})_{i=1}^d\\
    =& (\sum_{j=1}^d \frac{\partial \log p_Y(y) + \log(|det(A^{-1}|) }{\partial y_j} A_{ji})_{i=1}^d\\
    =& A^T \nabla_y \log p_Y(y)
\end{align*}

We can see that if we let $$\kk_y(y,y') = A \kk_x(x(y), x'(y')) A^T = A \kk_x(A^{-1}(y-b), A^{-1}(y'-b)) A^T,$$ we would have:
\begin{equation}
    A\phi_{\kk_x}^*(x) = \phi_{\kk_y}^*(y)
\end{equation}

Now $\kk_x = k_{\text{RBF}}\textbf{I}_D$, we will have:
\begin{align*}
    \kk_y(y,y') =& A \kk_x(A^{-1}(y-b), A^{-1}(y'-b)) A^T\\
    =& A \textbf{I}_D \exp\bigg\{-\|A^{-1}(y-y')\|^2/2h\bigg\} A^T \\
    =& (A A^T) \exp\bigg\{-(y-y')^T(A A^T)^{-1} (y-y') /2h\bigg\} \\
    =& \Sigma \exp\bigg\{-(y-y')^T\Sigma^{-1} (y-y') /2h\bigg\}
\end{align*}

For non-Gaussian target, we use $M_p$ to replace $\Sigma^{-1}$ and get our matrix kernel similar to Newton's method.
% , where we interpolate the geometry of the objective distribution is by taken a local kernel $k_j$ as:
% \begin{equation*}
%     k_j(x,x') = \exp\{(x-x^T)Q_j(x-x^T)\}
% \end{equation*}
% where $Q_j \approx \nabla^2 \log p(x_j)$, $x_j$ to be the center/random particles of local cluster $X_j$. The idea is firstly brought up at 'Stein Newton' paper.

% And for $B_j$ we can either pick $Q_j^{-1}$ as a natural gradient style, where we consider the norm of the space as $\|x\|^2 = x^T Q x$ and applying natural gradient over such norm space. Or let $B_j$ to be the covariance matrix for $X_j$.

\subsection{Constructing Matrix-Valued Kernels}
To start with the following basic results of RKHS. 
\begin{lem}
Assume $\H_0$ is a RKHS with matrix kernel $\vv K$. 

i) %If $\ff_0\in \H_0$ has matrix kernel $\vv K_0$, and 
Let $\H$ be the set of functions formed by $\ff(x) = \vv M(x) \ff_0(x)$, where $\ff_0\in\H$ and $\vv M(x)$ is a matrix-valued function. 
Then $\H$ is also an RKHS. It is matrix kernel is 
$$
 {\vv K}(x,x') = \vv M(x) {\vv K}_0(x,x')\vv M(x')^\top. 
$$

ii) Let $\H$ be the set of functions of form $\ff(x) = \ff_0(T(x))$, where 
$\ff_0\in \H$ and $T(x)$ is a one-to-one map on $\X$. 
Then $\H$ is a RKHS with kernel 
$$
 {\vv K}(x,x') = {\vv K}_0(T(x),T(x')). 
 %\vv M(x')^\top. 
 $$
%Let $T(x)$ be a one-to-one map
%$\ff_0\in \H_0$ has matrix kernel $\vv K_0$. 
\label{lem:transform_RKHS}
\end{lem}
\iffalse 
\begin{proof}
Note that $\H_0$ is the closure of functions of form 
$$
\ff_0(x) = \sum_{i} \vv K_0(x, x_i) \vv w_i,
$$
where $\{x_i\} \subseteq \X$ and $\{\vv w_i\} \in \RR^d$. In i), $\H$ is the closure of 
$$
\ff_0(x) = \sum_{i} \vv M(x) K_0(x, x_i)\vv w_i,...
$$
\end{proof}
\fi
%\end{}

This motivates a procedure to construct matrix kernels: 
given an existing matrix kernel $K_0$, (e.g., a diagonal kernel), 
and matrix function $M$ and one-to-one map $T(x)$. We have kernel 
%folowing general form of matrix kernel: 
$$
\vv K(\vx, \vx)  = \vv M(x) \vv K_0(T(x),T(x')) \vv M(x')^\top.
$$
It is the kernel of RKHS consisting of $M(x) \phi_0(T(x))$, $\forall \phi_0\in\H_0$. 

\subsection{SVGD under Change of Variables}
%%^Assume $$
We start with the following invariant property of Stein operator under
change of variables: %one-to-one maps
\begin{lem}
Let $p$ be a continuous differentiable density function and $p_0$ the distribution of $ x_0  = T(x)$ when $x\sim p$, where  $T$ is a continuous differentiable one-to-one map on $\X$.  We have 
$$
\E_{x\sim \rho} [\stein_{p}  \phi(x)] = \E_{ x_0 \sim \rho_0} [\stein_{ p_0} \phi_0 (x)]  
$$
where 
$$
%\tilde 
\phi(x) = (T'(x))^{-1}\phi_0(T(x)). 
$$
\end{lem}
Therefore,  via a one-to-one map $T$, the SVGD update on $p_0$ with kernel $\vv K_0$ is equivalent to (when step-size is infiteismal) SVGD update on $p$ with kernel 
$$
\vv K(\vx, \vx)  = ( T'(x))^{-1} \vv K_0(T(x),T(x')) ( T'(x'))^{-\top}.
$$
%
This implies a general approach to construct kernels. The idea is that we should construct transform $T$ to change $p$ to a easier-to-sample distribution $p$ for which a simple kernel can be constructed. Here are few examples: 

\begin{enumerate}
    % \item \red{How about $T(x) = H(x)^{-\frac{1}{2}}\nabla_x \log p(x)$}?
    \item Take $T(x) = \vv H(x)^{1/2} x$, where $\vv H(x) = \nabla_x^2 \log p(x)$ is the Hessian matrix. If $p$ is a multivariate Gaussian, then $T$ transforms $p$ to a Gaussian with identity covariance, for which linear kernel, or coordinate-wise kernel works best. 
    We have 
      $$
    \vv K(x,x') = 
     T'(x)^{-1} \vv K_0(\vv H(x)^{1/2}x, \vv H(x')^{1/2} x') T'(x')^{-\top}. 
    $$
    Assume $H(x)$ almost stays constant (so that $p$ is close to Gaussian), 
    and hence $T'(x)\approx \vv H(x)^{1/2}x$. We get
    %Consider 
    %$$
    %%T'(x) = \vv H(x)^{1/2} + \vv H'(x){1/2} x
%    $$
    %Then this motivates %we have 
    $$
    \vv K(x,x') = 
    \vv H(x)^{-1/2} \vv K_0(\vv H(x)^{1/2}x, \vv H(x')^{1/2} x') \vv H(x')^{-\top /2}. 
    $$
    This is a natural \textbf{Newton-version of SVGD}.  
    This kernel is a valid poisitive definite matrix kernel, despite not being  exactly the kernel derived using change of variable because $T(x)'$ does not equal $H(x)^{1/2}$. 
    What $K_0$ we should use?  There are few things we should try:
    \begin{enumerate}
            \item $\vv K_0$ could be a standard RBF kernel or linear kernel. 
        \item  $\vv K_0(x,x') = diag(k_i(x_i, x_i'))$. It is diagonal kernel, where $k_i$ is a one-dimensional RBF or linear kernel. 
        \item We can use linear combination of the above to make sure $\vv K_0$ is strictly positive definite. 
    \end{enumerate}

\item Could you try the following \textbf{mixture Hessian kernel}:
$$
\vv K(x,x') = \sum_i w_i(x) w_i(x') \vv K_i(x,x'), 
$$
where 
$$
\vv K_i(x,x') = H_i^{-1/2} K_0(H_i^{1/2}x, H_i^{1/2}x') H_i^{-\top/2},
$$
where $H_i$ is the Hessian at $x_i$ and $w_i(x)$ measures a closeness to $x_i$, which could equal $\exp(-\alpha ||x-x'||_{H_i}^2)$. 
    
\end{enumerate}



\subsection{Sum of Separable Kernel}
A more complex kernel can be written as sum of separable (SoS) kernel:
\begin{equation*}
    \kk(x,x') = \sum_{q=1}^{Q} k_q(x,x') B_q.
\end{equation*}

For this setting, following proposition \ref{pro:sep_svgd}, by linearity of expectation we have the optimum $\ff^*$ as:
\begin{equation}
    \ff_\kk^*(x) = \sum_{i=1}^{Q} B_q \ff_{k_q}^*(x),
\label{equ:sos_svgd}
\end{equation}
where $\ff_q^*(x)$ is the optimum update direction if we choose a scalar kernel $k_q$.

xxxx

\paragraph{Relation to Graphical-SVGD}
If we let number of different scalar kernel $Q = D$ and we let $B_q = e_q e_q^T$, we have: 
$$\kk(x,x')_{i,j} = \delta_{i,j} k_i(x,x'),$$
which is exactly as Graphical SVGD settings \cite{wang2018stein}

\paragraph{Relation to Stein variational Newton
method}
Graph SVGD \citep{xx} is a recently introduced xxx method that xx. Here, we show that graphical-SVGD can be derived from xxx with a xx kernel thatx, 
so that the velocity xx, in this case, Eq xxx becomes xxx


\subsection{SVGD with  Kronecker-factored Approximate Curvature}

Method that employ second order information
have the potential to speed up first order gradient 
descent by correcting for imbalanced curvature.
The parameters are then updated by
$$
\theta \leftarrow \theta -\eta G^{-1}\nabla_\theta R(\theta),
$$
where $\eta$ is a positive learning rate and $G$
is a preconditioning matrix capturing the local curvature
or related information such the Hessian matrix or the
Fisher Information matrix. Matrix $G$ has a size
of $n_\theta \times n_\theta$.


==> tex/mixture.tex <==
\section{Mixture Matrix Kernel}
We can apply mixture idea into designing the kernel, where we first cluster particles into several group, and update each group locally with a picked local kernel. The clustering process can also view as a probability to assign particles for each kernel. However, in computation we just calculate the gradient within final cluster to accelerate SVGD. (so $N^2$ into $\sum n_j^2$ if each cluster has $n_j$ particles)

\begin{algorithm}[t] 
\caption{Mixture Matrix Kernel SVGD} 
\label{alg:mixture_svgd}
\begin{algorithmic} 
\STATE {\bf Input:} initial particles $\{x_i\}_{i=1}^n$;
\FOR{iteration $t$}
\STATE Cluster $\{x_i\}_{i=1}^n$ into several groups $X_1, X_2, ..., X_m$, $X_j = \{x_1^{(j)}, ..., x_{n_j}^{(j)}\}$ with $n = \sum_{j=1}^m n_j$.
\STATE Do matrix kernel SVGD in each group $X_j$ with an appropriate scalar kernel $k_j$ and an appropriate PSD matrix $B_j$
\STATE Update by $x_i^{(j)} \gets x_i^{(j)} + \epsilon B_j \phi_j^*(x_i^{(j)})$
\ENDFOR
\end{algorithmic} 
\end{algorithm}

==> tex/moment_matching.tex <==

\section{Matrix Moment Matching for Gaussian Models}
In SVGD as moment matching paper \cite{liu2018stein}, 
we know that using a linear kernel we could exactly recover any second order function with $d+1$ points.
\red{Need to check the conclusion here}
% if we have a Gaussian target with $Q$ as inverse of covariance matrix, $\mu$ be the mean, then
% \begin{align*}
%     \stein_p k(x,x') = -Q(x-\mu)k(x,x') + \nabla_{x} k(x,x')
% \end{align*}
% For the fixed point solution $x_i^*$, we will have $\E_{x\sim \hat{\mu}}[\stein_p k(x,x_i^*)] = 0$. 
% On the other hand, we have stein identity that $\E_{x\sim p}[\stein_p \phi(x)] = 0$.
% So if $f(x)$ lies in linear span of $\{\stein_p k(x,x_i^*)\}$, we can estimate $f(x)$ accurately.
% Especially for second moment $f(x) = x^T x$.

% For linear kernel $k(x,x') = x^T x' + 1$, the linear span can be written as:
% \begin{align*}
%     &\sum_{i=1}^n a_i^T \stein_p k(x,x_i^*) + b_i\\
%     =&\sum_{i=1}^n 
% \end{align*}

Another interesting fact is that when the Gaussian is isotropic, i.e. the covariance matrix is diagonal, every dimension is independent. 
Thus we could estimate each dimension with a corresponding linear kernel $x_i x'_i +1$, to recover variance in each dimension exactly.
Since they are all independent, we can do the SVGD start at only $2$ points, to find the location that exactly recover variances in all dimension, i.e. the diagonal covariance matrix.

A general problem is that for non-isotropic Gaussian, if we want to exactly recover the variance for each dimension, i.e. the diagonal of the covariance matrix, 
can we use just two points to do so?

With the help of matrix kernel, the answer is yes. 
Suppose we have a distribution $p(x)\propto \exp\{-\frac{1}{2}(x-\mu)^T Q(x-\mu)\}$.
The intuition behind is that we left times a covariance matrix $B = Q^{-1}$
to cancel out the dependency of $Q$ from the gradient of $\log p(x)$.

To be more specific, 
% let our matrix kernel be
% \begin{align*}
%     \kk(x,y) = \sum_{j=1}^d e_j e_j^T B(x_j y_j + 1),
% \end{align*}
we have the following proposition:
\begin{pro}
The fixed points of SVGD with matrix kernel 
$$\kk = \sum_{j=1}^d e_j e_j^T B(x_j y_j + 1),$$ 
where $B$ is the covariance matrix of our target distribution,
can exactly recovers the variance for each dimension, i.e. the diagonal of the covariance matrix, when $rank(\Phi) \geq 2$.
Here $\Phi$ is a $(d+1)\times n$ matrix defined by
\[
\Phi = \left[
\begin{array}{cccc}
    x_1 & x_2 & ... & x_n \\
    1 & 1 & ... & 1
\end{array}
\right],
\]
with $x_1, x_2,...,x_n$ be the fixed points of SVGD.
\label{pro:matrix_moment}
\end{pro}


% \section{Experiment}
% We are going to test several environments with the following several different variational methods:
% \begin{enumerate}
%     \item Vanilla SVGD with median kernel trick. Here we set the kernel to be a scalar RBF kernel with median distance as bandwidth.
%     \item SVGD with scalar average Hessian kernel, where
%     \begin{equation*}
%         k(x,x') = \exp(-\frac{1}{2}(x-x')^T Q(x-x')),
%     \end{equation*}
%     with Q be the average Hessian of $\log p$. Specifically, if the target is a gaussian, $Q$ would be the inverse of its covariance matrix.
%     \item Matrix kernel SVGD with RBF kernel. The PSD matrix $B$ we choose to be inverse of $Q$, in the sense that we are doing natural gradient descend under norm space defined by $\|x\|_Q = x^T Qx$.
%     \item Combining 2,3, where we take matrix kernel $B = Q^{-1}$ and average Hessian kernel.
%     \item Mixture Matrix kernel, with local matrix kernel for each cluster of the current particles.
% \end{enumerate}
% In figure, we will use \textbf{Vanilla SVGD, SVGD Hessian, Matrix SVGD, Matrix SVGD Hessian, Mixture Matrix SVGD} to indicate the above methods.

% \subsection{Plan of experiment}
% \begin{enumerate}
%     \item We expect that methods 3,4 can accelerate learning rate under ill-conditioned matrix $Q$, where gradient descend would be slow as the curvature of distribution is skew. We will show that by testing over the Gaussian distribution with covariance matrix $\Sigma$ taken with condition number from 1 to 100.
%     \item We expect that method 2,4,5 can learn the shape better, leading a better estimation of variance and other high moment function. We will show that by testing over mixture model and other Bayesian inference task. We expect 5 will do best for mixture model, when the clustering is good enough.
% \end{enumerate}

% \subsection{Gaussian}
% We set the target distribution as multivariate Gaussian with:
% \begin{equation*}
%     p(x) \propto \exp\{-\frac{1}{2}(x-\mu)^T Q (x-\mu)\}
% \end{equation*}
% with $Q = \Sigma ^{-1}$ as a (sparse) PSD matrix, similar setting as Graphical SVGD settings, except that we here set the graph as a sparse random graph with each edge occurs with probability $1/d$(d is the dimension, or the total number of nodes in graph).

% We inherit the adaptive step size with Adagrad for all four methods.

% Result for first and second moment estimation, where $y-axis$ is log MSE.

% \subsubsection{2D-gaussian}
% We construct skew covariace matrix $\Sigma$ by
% $$
% \Sigma = P^T D P
% $$
% with 
% $P = \left[\begin{array}{cc}cos(\theta) & -sin(\theta) \\ sin(\theta) & cos(\theta)\end{array}\right]$, and $D=\left[\begin{array}{cc}1 & 0 \\ 0 & \frac{1}{\kappa}\end{array}\right]$ as a diagonal matrix with condition number $\kappa$.
% We test the first four algorithms with condition number $\kappa$ from $1$ to $100$, compared with the number of steps each algorithm need to converge to the accuracy as simple Monte Carlo achieve. Figure 
% \begin{figure*}
% \centering
% \begin{tabular}{ccc}
% \label{fig:gau2D}
% \raisebox{3.0em}{\rotatebox{90}{\scriptsize \# iteration}}
% \includegraphics[height = 0.35\textwidth]{figure/gaussian/condition_number.png}&
% \raisebox{3.0em}{\rotatebox{90}{\scriptsize log MSE}}
% \includegraphics[height = 0.35\textwidth]{figure/gaussian/Ex.png} \\
% condition number & \# iteration 
% \end{tabular}
% \caption{2D-Gaussian: number of particles = 100, dimension = 2. with best step size}
% \end{figure*}

% \subsubsection{High-dimensional Gaussian}
% Need to figure why Natural with Hessian kernel is not as good as RBF kernel
% \begin{figure*}
% \centering
% \begin{tabular}{cc}
% \raisebox{3.0em}{\rotatebox{90}{\scriptsize log MSE}}
% \includegraphics[width=0.45\textwidth]{figure/high-dimension/EX_gau_d40.png} &
% \includegraphics[width=0.45\textwidth]{figure/high-dimension/EX2_gau_d40.png}
% \end{tabular}
% \caption{High-dimensional Gaussian: number of particles = 100, dimension = 40. with best step size}
% \end{figure*}

% \subsection{Gaussian Mixture}
% \begin{figure*}
% \centering
% \begin{tabular}{ccc}
% \raisebox{2.0em}{\rotatebox{90}{\scriptsize Vanilla SVGD}}
% \includegraphics[width=0.3\textwidth]{figure/gau_mix/SVGD/iter=0.pdf} &
% \includegraphics[width=0.3\textwidth]{figure/gau_mix/SVGD/iter=100.pdf} &
% \includegraphics[width=0.3\textwidth]{figure/gau_mix/SVGD/iter=200.pdf} \\
% iter = 0 & iter = 100 & iter = 200\\
% \raisebox{2.8em}{\rotatebox{90}{\scriptsize SVGD H}}
% \includegraphics[width=0.3\textwidth]{figure/gau_mix/SVGDh/iter=0.pdf} &
% \includegraphics[width=0.3\textwidth]{figure/gau_mix/SVGDh/iter=100.pdf} &
% \includegraphics[width=0.3\textwidth]{figure/gau_mix/SVGDh/iter=200.pdf} \\
% iter = 0 & iter = 100 & iter = 200\\
% \raisebox{1.7em}{\rotatebox{90}{\scriptsize Natural SVGD}}
% \includegraphics[width=0.3\textwidth]{figure/gau_mix/nSVGD/iter=0.pdf} &
% \includegraphics[width=0.3\textwidth]{figure/gau_mix/nSVGD/iter=100.pdf} &
% \includegraphics[width=0.3\textwidth]{figure/gau_mix/nSVGD/iter=200.pdf} \\
% iter = 0 & iter = 100 & iter = 200\\
% \raisebox{1.5em}{\rotatebox{90}{\scriptsize Natural SVGD H}}
% \includegraphics[width=0.3\textwidth]{figure/gau_mix/nSVGDh/iter=0.pdf} &
% \includegraphics[width=0.3\textwidth]{figure/gau_mix/nSVGDh/iter=100.pdf} &
% \includegraphics[width=0.3\textwidth]{figure/gau_mix/nSVGDh/iter=200.pdf} \\
% iter = 0 & iter = 100 & iter = 200\\
% \end{tabular}
% \caption{Gaussian Mixture 2D, shape evolution, with 200 particles}
% \end{figure*}

% \begin{figure*}
% \centering
% \begin{tabular}{cc}
% \raisebox{3.0em}{\rotatebox{90}{\scriptsize log MSE}}
% \includegraphics[width=0.45\textwidth]{figure/gau_mix/EX.png} &
% \includegraphics[width=0.45\textwidth]{figure/gau_mix/EX2.png} 
% \end{tabular}
% \caption{Gaussian Mixture 2D: number of particles = 200. with best step size}
% \end{figure*}

% Need to find out when does it work for Gaussian mixture in high dimension
% \subsection{Double Banana}
% \begin{figure*}
% \centering
% \begin{tabular}{cccc}
% \raisebox{1.0em}{\rotatebox{90}{\scriptsize Vanilla SVGD}}
% \includegraphics[width=0.23\textwidth]{figure/banana/SVGD/iter=0.pdf} &
% \includegraphics[width=0.23\textwidth]{figure/banana/SVGD/iter=10.pdf} &
% \includegraphics[width=0.23\textwidth]{figure/banana/SVGD/iter=20.pdf} &
% \includegraphics[width=0.23\textwidth]{figure/banana/SVGD/iter=30.pdf} \\
% iter = 0 & iter = 10 & iter = 20 & iter = 30\\
% \raisebox{1.8em}{\rotatebox{90}{\scriptsize SVGD H}}
% \includegraphics[width=0.23\textwidth]{figure/banana/SVGDh/iter=0.pdf} &
% \includegraphics[width=0.23\textwidth]{figure/banana/SVGDh/iter=10.pdf} &
% \includegraphics[width=0.23\textwidth]{figure/banana/SVGDh/iter=20.pdf} &
% \includegraphics[width=0.23\textwidth]{figure/banana/SVGDh/iter=30.pdf} \\
% iter = 0 & iter = 10 & iter = 20 & iter = 30\\
% \raisebox{0.8em}{\rotatebox{90}{\scriptsize Natural SVGD}}
% \includegraphics[width=0.23\textwidth]{figure/banana/nSVGD/iter=0.pdf} &
% \includegraphics[width=0.23\textwidth]{figure/banana/nSVGD/iter=10.pdf} &
% \includegraphics[width=0.23\textwidth]{figure/banana/nSVGD/iter=20.pdf} &
% \includegraphics[width=0.23\textwidth]{figure/banana/nSVGD/iter=30.pdf} \\
% iter = 0 & iter = 10 & iter = 20 & iter = 30\\
% \raisebox{0.6em}{\rotatebox{90}{\scriptsize Natural SVGD H}}
% \includegraphics[width=0.23\textwidth]{figure/banana/nSVGDh/iter=0.pdf} &
% \includegraphics[width=0.23\textwidth]{figure/banana/nSVGDh/iter=10.pdf} &
% \includegraphics[width=0.23\textwidth]{figure/banana/nSVGDh/iter=20.pdf} &
% \includegraphics[width=0.23\textwidth]{figure/banana/nSVGDh/iter=30.pdf} \\
% iter = 0 & iter = 10 & iter = 20 & iter = 30\\
% \end{tabular}
% \caption{Double Banana, shape evolution, with 1000 particles}
% \end{figure*}

